Bootstrapping Graph Convolutional Neural Networks for Autism Spectrum Disorder Classification

Using predictive models to identify patterns that can act as biomarkers for different neuropathoglogical conditions is becoming highly prevalent. In this paper, we consider the problem of Autism Spectrum Disorder (ASD) classification where previous work has shown that it can be beneficial to incorporate a wide variety of meta features, such as socio-cultural traits, into predictive modeling. A graph-based approach naturally suits these scenarios, where a contextual graph captures traits that characterize a population, while the specific brain activity patterns are utilized as a multivariate signal at the nodes. Graph neural networks have shown improvements in inferencing with graph-structured data. Though the underlying graph strongly dictates the overall performance, there exists no systematic way of choosing an appropriate graph in practice, thus making predictive models non-robust. To address this, we propose a bootstrapped version of graph convolutional neural networks (G-CNNs) that utilizes an ensemble of weakly trained G-CNNs, and reduce the sensitivity of models on the choice of graph construction. We demonstrate its effectiveness on the challenging Autism Brain Imaging Data Exchange (ABIDE) dataset and show that our approach improves upon recently proposed graph-based neural networks. We also show that our method remains more robust to noisy graphs.

==> graph.tex <==
In this section we briefly introduce convolutional neural networks on graphs, and present our bootstrapped training strategy using an ensemble of randomized population graphs.
\subsection{Graph Convolutional Neural Networks}
Convolutional neural networks enable extraction of statistical features from structured data, in the form of local stationary patterns, and their aggregation for different semantic analysis tasks, e.g. image recognition or activity analysis. When the signal of interest does not lie on a regular domain, for example graphs, generalizing CNNs is particuarly challenging due to the presence of convolution and pooling operators, typically defined on regular grids. 

In graph signal processing theory, this challenge is alleviated by switching to the spectral domain, where the convolution operations can be viewed as simple multiplications. In general, there exists no mathematical definition for the translation operation on graphs. However, a spectral domain approach defines the localization operator on graphs via convolution with a Kronecker delta signal. However, localizing a filter in the spectral domain requires the computation of the graph Fourier transform and hence translations on graphs are computationally expensive. We refer the reader to \cite{Kipf2016GCNN, Defferrard2016GCNN} for a detailed description of graph convolutional neural network architectures. 

%Before we describe the graph CNN architecture used in our approach, we define the Fourier transform for signals on graphs.

%\vspace{0.1in}
%
%\noindent \textbf{Preliminaries:} Formally, an undirected weighted graph is represented by $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathbf{W})$, where $\mathcal{V}$ denotes the set of vertices or nodes, $\mathcal{E}$ denotes the set of edges and $\mathbf{W}$ is the adjacency matrix that specifies the weights between edges $\mathbf{W}_{ij}, \forall e_i, e_j \in \mathcal{E}$. The fundamental component of graph analysis is the normalized graph Laplacian $\mathbf{L}$, which is defined as $\mathbf{I} - \mathbf{D}^{-1/2}\mathbf{W} \mathbf{D}^{-1/2}$, where $\mathbf{D}_{ii} = \sum_j \mathbf{W}_{ij}$ is the degree matrix and $\mathbf{I}$ denotes the identity matrix. The set of eigenvectors of the Laplacian are referred to as the graph Fourier basis, $\mathbf{L} = \mathbf{U} \mathbf{\Lambda} \mathbf{U}^T$, and hence the Fourier transform of a signal $\mathbf{x} \in \mathbb{R}^N$ is defined as $\mathbf{U}^T \mathbf{x}$. Finally, the spectral filtering operation can be defined as $\mathbf{y} = g_{\theta}(\mathbf{L}) \mathbf{x} = \mathbf{U} g_{\theta}(\mathbf{\Lambda}) \mathbf{U}^T\mathbf{x} $, where $g_{\theta}$ is the parametric filter.
%
%\vspace{0.1in}
%
%\noindent \textbf{Formulation:} Since spectral filtering is computationally prohibitive as the number of nodes in the graph increases, \cite{Hammond2011} proposed to approximate $g_{\theta}(\mathbf{\Lambda})$ as a truncated expansion in terms of the Chebyshev polynomials recursively.
%
%\begin{equation}
%g_{\hat{\theta}}(\mathbf{\Lambda}) \approx \sum_{k=0}^K \hat{\theta}_k T_k(\tilde{\mathbf{\Lambda}}),
%\end{equation}where $\hat{\theta}$ is the set of Chebyshev coefficients, $K$ is the order for the approximation, $\tilde{\mathbf{\Lambda}}$ are rescaled eigenvalues and the Chebyshev polyomials $T_k(x)$ are recursively defined as $2xT_{k-1}(x) - T_{k-2}(x)$. Using this approximation in the spectral filtering operation implies that the filtering is $K-$localized, i.e., the filtering depends only on the $K$ neighborhood nodes. We can use this K-localized filtering to define convolutional neural networks on graphs.
%
%For example, the approach in \cite{Kipf2016GCNN} uses $K=1$ such that the layer-wise computation is linear w.r.t $\mathbf{L}$. Though, this is a crude approximation, by stacking multiple layers one can still recover a large class of complex filter functions, that are not just limited to the linear functions supported by the first order Chebyshev approximation. The resulting filtering can then be expressed as
%\begin{equation}
%g_{\hat{\theta}} \star \mathbf{x} = \hat{\theta}_0 \mathbf{x} - \hat{\theta}_1 \mathbf{D}^{-1/2}\mathbf{W} \mathbf{D}^{-1/2} \mathbf{x}.
%\end{equation}Here, $\star$ indicates the convolution operation in the spatial domain. Note that, the filter parameters are shared over the whole graph. In summary, the complete processing in a layer is defined as follows: Given an input function $\mathbf{X} \in \mathbb{R}^{T \times N}$, where $T$ is the number of nodes, and $N$ is the dimension of the multivariate function at each node, the activations can be computed as
%\begin{equation}
%\sigma(\tilde{\mathbf{D}}^{-1/2} \tilde{\mathbf{W}}\tilde{\mathbf{D}}^{-1/2} \mathbf{X} \mathbf{\Theta}).
%\end{equation}Here $\mathbf{\Theta} \in \mathbb{R}^{N \times F}$ is the set of filter parameters, the graph Laplacian is reparameterized as 
%$\tilde{\mathbf{D}}^{-1/2} \tilde{\mathbf{W}}\tilde{\mathbf{D}}^{-1/2} = \mathbf{I} + \mathbf{D}^{-1/2} \mathbf{W}\mathbf{D}^{-1/2}$. The activation function $\sigma$ is chosen to be ReLU in our implementation. This linear formulation of graph convolutional networks is much more computationally efficient compared to the accurate filtering implementation. 

\subsection{Ensemble Learning}
As described in the previous section, population graphs provide a convenient way to incorporate non-imaging features into the predictive modeling framework, where the connectivity features from fMRI data are used as a function on the graph. While G-CNN can automatically infer spectral filters for achieving  discrimination across different classes, the sensitivity of its performance to the choice of the population graph is not straightforward to understand. Consequently, debugging and fine-tuning these networks can be quite challenging. 

The conventional approach to building robust predictive models is to infer an ensemble of weak learners from data and then fuse the decisions using a consensus strategy. The need for ensemble models in supervised learning has been well-studied \cite{Dietterich2000}. A variety of bootstrapping techniques have been developed, wherein multiple weak models are inferred using different random subsets of data. The intuition behind the success of this approach is statistical, whereby different models may have a similar training error when learned using a subset of training samples, but their performance on test data can be different since they optimize for different regions of the input data space. 

We employ a similar intuition to building models with population graphs, wherein the quality of different similarity metrics for graph construction can lead to vastly different predictive models. More specifically, starting with a population graph, we create an ensemble of graphs, $\{\mathcal{G}_p\}_{p=1}^P$, by dropping out a pre-defined factor of edges randomly. In this paper, we use a uniform random distribution for the dropout, though more sophisticated weighted distributions could be used. For each of the graphs in the ensemble, we build a G-CNN model (details in Section \ref{sec:results}) with the connectivity features as the $N-$dimensional multivariate function at each node. The output of each of the networks is a softmax function for each node, indicating the probability for the subject to be affected by ASD. Note that, unlike conventional ensemble learners, we do not subsample data, but only subsample edges of the population graph. Given the decisions from all the weak learners, we employ simple consensus strategies such as averaging or obtaining the maximum of the probabilities estimated by each of the G-CNNs for a test subject. As we will show in our experimental results with the ABIDE dataset, the proposed ensemble approach boosts the performance of all the population graph construction strategies discussed in Section \ref{sec:approach}.

